A Representation-Independent Second-Moment Barrier for Nonadaptive Cyclic-Forrelation Estimators

Cyclic Forrelation asks for the normalized trace $T_k$ of $k$ Boolean phase oracles on $\mathbb{F}_2^n$, alternating with $n$-qubit Hadamard transforms, where $N=2^n$. For every nonadaptive estimator with budgets $q_1,\ldots,q_k$, arbitrarily correlated query sets, and arbitrary nonlinear postprocessing, we prove $\mathbb{E}_{R,f}[G_R(f)^2]\ge N^{k-2}\mathsf{Corr}(h,T_k)^2/\prod_{j=1}^{k}q_j$, with constant $1$ attained by Horvitz--Thompson Cartesian-product sampling. The proof projects each fixed transcript onto full-degree Walsh monomials and applies weighted Cauchy--Schwarz against an exact coverage budget. Thus the Cartesian scale $N^{1-2/k}$ is unavoidable when uniform target overlap and second moment are both bounded; unbiasedness alone gives no such restriction because a one-probe correction can restore it with heavy-tailed output. Separately, we construct a six-oracle complementary-subspace ensemble satisfying $W_6=\sigma I$ and an exact matching-certificate coupling, but give a certified adaptive algorithm recovering $\sigma$ in $n^{O(1)}N^{1/4}$ queries. These results delimit two approaches to the odd-cycle nonadaptive gap and the $\Omega(N^{1/4})$ adaptive lower bound; they do not close either gap for worst-case constant-error estimation or for a new hard distribution.

==> template_core/color_tokens.tex <==
\RequirePackage{xcolor}
\definecolor{PaperInk}{HTML}{18232B}             % neutral blue-black ink
\definecolor{PaperMutedInk}{HTML}{5B6873}        % cool gray-blue
\definecolor{PaperRule}{HTML}{D1D8DE}            % quiet rule gray
\definecolor{PaperAccent}{HTML}{003155}          % Prussian Blue: primary structure
\definecolor{PaperAccentDark}{HTML}{00223D}      % dark Prussian Blue
\definecolor{PaperAccentLight}{HTML}{E6EEF3}     % pale Prussian wash
\definecolor{PaperAccentPale}{HTML}{F6F9FB}      % paper-white blue wash
\definecolor{PaperNavigation}{HTML}{1B3F8D}      % Mingjing Blue: headings/links
\definecolor{PaperNavigationLight}{HTML}{E9EEFA} % pale Mingjing wash
\definecolor{PaperDefinition}{HTML}{244117}      % Corn: secondary semantic accent
\definecolor{PaperDefinitionLight}{HTML}{EEF2EA} % pale Corn wash
\definecolor{PaperGold}{HTML}{C79C5E}            % Champagne Gold: sparse accent
\definecolor{PaperGoldLight}{HTML}{FAF3E8}       % pale Champagne wash
\definecolor{PaperAlgorithmLight}{HTML}{F0F5F8} % algorithm body wash
\definecolor{PaperLink}{HTML}{1B3F8D}            % internal references
\definecolor{PaperCitation}{HTML}{244117}        % citations
\definecolor{PaperUrl}{HTML}{003155}             % external URLs
\definecolor{PaperDraft}{HTML}{9A4F3D}           % restrained warm draft marker


==> template_core/layout.tex <==
\RequirePackage[margin=0.9in]{geometry}
\linespread{1.05}
\frenchspacing
\widowpenalty=10000
\clubpenalty=10000
\setlength{\emergencystretch}{3em}
\setlength{\parindent}{1.2em}
\setlength{\parskip}{0pt}


==> template_core/typography.tex <==
\RequirePackage{iftex}
\ifPDFTeX
  \RequirePackage[T1]{fontenc}
  \RequirePackage[utf8]{inputenc}
  \RequirePackage{lmodern}
\else
  \RequirePackage{fontspec}
  \setmainfont{Latin Modern Roman}
  \setsansfont{Latin Modern Sans}
  \setmonofont{Latin Modern Mono}
\fi
\newcommand{\PaperBodyFont}{\rmfamily}
\newcommand{\PaperHeadingFont}{\sffamily}
\newcommand{\PaperCaptionFont}{\sffamily}
\newcommand{\PaperCodeFont}{\ttfamily}

